One2Any: One-Reference 6D Pose Estimation for Any Object

6D object pose estimation remains challenging for many applications due to dependencies on complete 3D models, multi-view images, or training limited to specific object categories. These requirements make generalization to novel objects difficult for which neither 3D models nor multi-view images may be available. To address this, we propose a novel method One2Any that estimates the relative 6-degrees of freedom (DOF) object pose using only a single reference-single query RGB-D image, without prior knowledge of its 3D model, multi-view data, or category constraints. We treat object pose estimation as an encoding-decoding process, first, we obtain a comprehensive Reference Object Pose Embedding (ROPE) that encodes an object shape, orientation, and texture from a single reference view. Using this embedding, a U-Net-based pose decoding module produces Reference Object Coordinate (ROC) for new views, enabling fast and accurate pose estimation. This simple encoding-decoding framework allows our model to be trained on any pair-wise pose data, enabling large-scale training and demonstrating great scalability. Experiments on multiple benchmark datasets demonstrate that our model generalizes well to novel objects, achieving state-of-the-art accuracy and robustness even rivaling methods that require multi-view or CAD inputs, at a fraction of compute.

==> supp_sec/1_training_details.tex <==
\section{Training Details}
\label{sec:training_details}
We describe the training process of our model, including the preprocessing of the data, and the network architecture details.
% which builds on the strengths of pre-trained architectures while incorporating specific modifications to generate ROC maps optimized for pose prediction tasks. To enhance training efficiency and address the unique characteristics of ROC maps compared to standard RGB images, the decoder is trained from scratch. The resulting OPD module efficiently generates ROC maps aligned with the reference coordinate system, enabling robust object pose estimation across diverse viewpoints. Throughout both the main text and the supplementary material, ROC maps are represented by their final output point clouds,  $Y_Q$  or  $Y_A$ , despite being parametrized by image pixel locations.

\subsection{Preprocessing of the Data }
We begin by masking each object in the image, cropping it so the object is centered, and resizing it to a resolution of  $192\times 192$. 

\noindent{}\textbf{Scale matrix $\mathbf{S}$. } The scale matrix $\mathbf{S}$ is obtained from the reference image $A$. The computation of the scale matrix $\mathbf{S}$  is detailed here. Let  $d^{A_D}$ represent the depth values in $A_D$, and $\begin{bmatrix} u \\ v \end{bmatrix} ^{A_D}$ denote the corresponding pixel positions of the object, pre-filtered using the mask $A_M$. The corresponding 3D point in the camera coordinate space for each pixel in the image  A  is given as $\begin{bmatrix} x \\ y \\ z \end{bmatrix} \in \mathbb{R}^3$.  Using this, we construct a point cloud$P_A \in \mathbb{R}^{N\times 3}$  where  $N$  is the number of points, computed as $N = \sum_{u}\sum_{v}{Q_M(u,v)=1}$.

To normalize the points into ROC space,  we apply the scale matrix $\mathbf{S}$, as defined in Equation \ref{eq:scale}. For each instance in the reference image, we establish a Reference Object Coordinate (ROC).

\begin{align}
\label{eq:scale}
        w = \operatorname{max}(\operatorname{max}(\begin{bmatrix} x \\ y \\z \end{bmatrix}^{P_A}) &- \operatorname{min}(\begin{bmatrix} x \\ y \\z \end{bmatrix}^{P_A}))\\
    c = \begin{bmatrix} c_x \\ c_y \\c_z \end{bmatrix}^{P_A} = (\operatorname{max}(\begin{bmatrix} x \\ y \\z \end{bmatrix}^{P_A})& + \operatorname{min}(\begin{bmatrix} x \\ y \\z \end{bmatrix}^{P_A})) / 2 \\
     Y_A = (Y_A - c) &/ (w \times 1.1) 
     % {p_A}^{\mathbb{O}} & += 0.5\\
    \end{align}
By determining the size scalar $w$ and the center $c$ of the point cloud $P_A$, we translate $P_A$ to the origin with the offset $c$ and scale it with $w \times 1.1$ to ensure all points lie within $[-0.5, 0.5]$. The result is the normalized 3D point cloud ${P_A}$ in ROC space, which is then mapped into an RGB image $Y_A$, referred to as the ROC map, where the RGB channels encode the 3D ROC positions.
%In detail, we find the maximum size $w^{P_A}$ and the center $c^{P_A}$ of the point cloud $P_A$, and we just move $P_A$ to the origin in the camera coordinate and scale it with $ 1 / (w^{P_A} \times 1.1)$ to make sure all points are within [-0.5, 0.5], and in the end move to [0,1] space.

In this process, the scale and shift transformation matrix $\mathbf{S}$ is also computed and recorded for further alignment on the predicted ROC map from the test image.
\begin{align}
     s &= 1 / (w \times 1.1) \\
     t &=  -1 \times c / s\\
     \mathbf{S} &= 
        {\begin{bmatrix}
     s & 0 & 0  & t_x\\
    0 &  s & 0 &t_y\\
   0 & 0 &  s & t_z \\
   0 & 0 & 0 & 1\\
\end{bmatrix}}
\end{align}

\subsection{Network Architecture}
\textbf{Diffusion Model \cite{rombach2022high}. } The text-to-image diffusion model is a generative framework designed to create high-quality images from textual descriptions. Its architecture consists of three key modules: an encoder and a decoder, based on VQVAE \cite{esser2021taming}, which map features between the image and latent spaces, and a U-Net module that performs denoising within the latent space. The diffusion proves its strong capability in image generation, and it can also cooperate with other generation tasks like depth generation \cite{ke2024repurposing}. Here, we extend the diffusion model to predict ROC maps. To improve time efficiency, we employ a feedforward stable diffusion model instead of the traditional iterative denoising process.

Following \cite{cai2024ov9d}, we utilize the stable diffusion model \cite{rombach2022high}, pre-trained on Laion-5b \cite{schuhmann2022laion}. We freeze the VQVAE module to encode the input query image $Q_{I}$, mapping it to the latent space as the feature map $\mathcal{F}^Q$. The U-Net is fine-tuned using our data pairs. Reference RGBD images serve as conditional inputs, processed through the Reference Object Encoder (ROE) and passed into the U-Net as feature maps  $\mathcal{F}^{A}$. The two feature embeddings $\mathcal{F}^Q$ and $\mathcal{F}^A$ , are integrated via the cross-attention modules in U-Net, producing the semantic and spatially aligned feature map $\mathcal{F}^{Q2A}$.  Since ROC maps differ significantly from typical RGB images, we train the decoder from scratch. The decoder progressively refines $\mathcal{F}^{Q2A}$  to reconstruct a high-resolution output aligned with the original image dimensions. The individual modules are detailed below.

\noindent{}\textbf{VQVAE. } We adopt the pre-trained VQVAE module from \cite{rombach2022high} and freeze it during training. Input images are normalized for better feature extraction.

\noindent{}\textbf{U-Net. } The U-Net is initialized with pre-trained weights from \cite{rombach2022high}. During the feedforward pass, no noise is added, allowing the U-Net to directly output meaningful feature embeddings. The ROE features serve as conditional inputs to the U-Net, interacting with the latent feature $\mathcal{F}^{Q}$ through cross-attention layers. The U-Net gradually learns to process the feature maps from ROPE and the test image.

\noindent{}\textbf{ROE.} The Reference Object Encoder (ROE), denoted as  $f(A; \theta_A)$  extracts latent encodings from a channel-wise concatenation of the reference RGB image, ROC map, and object mask. This encoding captures both texture and geometric information. The ROE processes these inputs through three convolutional layers with batch normalization and ReLU activation. A residual connection block \cite{he2016deep} further refines the features embeddings. The resulting feature maps are tokenized into patches with positional embeddings \cite{alexey2020image}, effectively guiding ROC map generation and maintaining fidelity to reference data, even under occlusion.

\noindent{}\textbf{Decoder.} The decoder consists of five convolutional layers with residual connections \cite{he2016deep}. Each layer includes a bilinear upsampling module to produce the final ROC map  $\hat{Y}_{Q}$. The decoder is initialized using Kaiming Initialization \cite{he2015delving}.


==> supp_sec/2_more_experimental_results.tex <==
\section{Experimental Results}
\label{sec:experimental_results}
In this section, we provide a detailed analysis of the experimental results and investigate the impact of training data scale on the performance of our model.

\subsection{Full Test Results on the YCB-Video Dataset}
We present the detailed test results on the YCB-Video \cite{xiang2017posecnn} test set in Table \ref{tab:ycbv_data_full}, including performance metrics for each object. For all one-view methods, only the first test image is used as the reference image. In contrast, multi-view-based methods such as FS6D \cite{he2022fs6d}, Predator \cite{huang2021predator}, and LoFTR \cite{sun2021loftr} are fine-tuned on the test set, following the protocol outlined in FS6D \cite{he2022fs6d}. Specifically, FS6D divides the test objects into three groups, training on two groups while testing on the remaining one. Our method demonstrates superior performance compared to other one-view-based approaches, particularly for the ADD metric, where it significantly outperforms all competing methods. Our method even surpasses some multi-view approaches that employ fine-tuning on the test data.


\begin{table*}[]
    \centering
    \footnotesize
       \setlength{\tabcolsep}{0.2mm}
    \caption{Performance on occluded YCB-Video \cite{xiang2017posecnn} dataset. We compare with point cloud registration methods, multi-view methods, and one-view methods. Predator \cite{huang2021predator}, LoFTR \cite{sun2021loftr} and FS6D \cite{he2022fs6d} are fine-tuned on the YCB-Video dataset. We evaluate ADD-S AUC and ADD AUC metrics. Results of multi-view methods are adopted from \cite{wen2024foundationpose}. For one-view methods, we provide the first image in the test set as the reference. The best performance among multi-view methods and one-view methods are highlighted in bold.}
    % \vspace{-0.3cm}
    \begin{tabular}{c| c c | c c |c c |c c || c c | c c | c c | c c}
    \toprule
        Methods  &\multicolumn{2}{c|}{\textbf{PREDATOR} \cite{huang2021predator}} & \multicolumn{2}{c|}{\textbf{LoFTR}\cite{sun2021loftr}} &  \multicolumn{2}{c|}{\textbf{FS6D} \cite{he2022fs6d}} & \multicolumn{2}{c||}{\textbf{FoundationPose} \cite{wen2024foundationpose}} &  \multicolumn{2}{c|}{\textbf{FoundationPose}\cite{wen2024foundationpose}} &  \multicolumn{2}{c|}{\textbf{Oryon} \cite{corsetti2024open}} &  \multicolumn{2}{c|}{\textbf{NOPE} \cite{nguyen2024nope}} & \multicolumn{2}{c}{\textbf{One2Any(Ours)}} \\
  
        Ref. Images & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{16 - CAD}  & \multicolumn{2}{c|}{1 - CAD} & \multicolumn{2}{c|}{1} & \multicolumn{2}{c|}{1 + GT trans} & \multicolumn{2}{c}{1} \\
        \midrule
        metrics & ADD-S & ADD & ADD-S & ADD  & ADD-S & ADD  & ADD-S & ADD & ADD-S & ADD & ADD-S & ADD & ADD-S & ADD & ADD-S & ADD \\
        \midrule
       002\_master\_chef\_can  &73.0 & 17.4 & 87.2 & 50.6& 92.6 & 36.8 & \textbf{96.9} & \textbf{91.3} &87.3 & 73.3 &  12.2 & 8.7 & 96.8 & 17.8 & \textbf{94.9} & \textbf{84.3}\\
003\_cracker\_box & 41.7 & 8.3 & 71.8 & 25.5  & 83.9 & 24.5 & \textbf{97.5} & \textbf{96.2} & \textbf{92.0}	& 72.2 &  6.5 & 3.3 & 83.0 & 2.8 & 91.1 & \textbf{83.3}\\
004\_sugar\_box &  53.7 & 15.3 & 63.9 & 13.4 & 95.1 & 43.9 & \textbf{97.5} & \textbf{87.2} &  88.2	&87.1 &  5.3 & 3.8 & 86.5 & 22.3 & \textbf{95.3} &\textbf{88.0} \\
005\_tomato\_soup\_can & 81.2 & 44.4 & 77.1 & 52.9 & 93.0 & 54.2 & \textbf{97.6} & \textbf{93.3} & 95.2 &	\textbf{92.3} & 10.9 & 5.9  & \textbf{95.9} & 48.4  & 93.6 & 80.9 \\
006\_mustard\_bottle &  35.5 & 5.0 & 84.5 & 59.0&  97.0 & 71.1 & \textbf{98.4} & \textbf{97.3} & 88.4 &	76.6 &  5.5 & 4.7 & 91.3 & 42.7 & \textbf{93.8} & \textbf{87.6}\\
007\_tuna\_fish\_can &  78.2 & 34.2 & 72.6 & 55.7 & 94.5 & 53.9 & \textbf{97.7} & \textbf{73.7} & 90.5 &	76.9 &23.2 & 15.6 &\textbf{97.0} & 33.3 & \textbf{95.9} & \textbf{90.0}\\
008\_pudding\_box &  73.5 & 24.2 & 86.5 & 68.1& 94.9 & 79.6 & \textbf{98.5} & \textbf{97.0} & 91.7 &	77.8 & 1.3 & 1.3 & 84.4 & 20.9 & \textbf{96.1} & \textbf{93.3} \\
009\_gelatin\_box &  81.4 & 37.5 & 71.6 & 45.2 & 98.3 & 32.1 & \textbf{98.5} & \textbf{97.3} & 92.7& 87.7 & 1.3 & 1.3 & 87.3 & 35.3 & \textbf{97.7} & \textbf{96.1}\\
010\_potted\_meat\_can &  62.0 & 20.9 & 67.4 & 45.1 & 87.6 & 54.9 & \textbf{96.6} & \textbf{82.3} & 90.3 & \textbf{83.5} & 38.9 & 19.2 & \textbf{92.8} & 31.9 & 86.3 &  72.5\\
011\_banana &  57.7 & 9.9 & 24.2 & 1.6 & 94.0 & 69.1 & \textbf{98.1} & \textbf{95.4} &90.3	& 76.3 & 4.9 & 4.1 & 61.3 & 11.4 & \textbf{95.0} & \textbf{85.7}\\
019\_pitcher\_base &  83.7 & 18.1 & 58.7 & 22.3 & 91.1 & 40.4 & \textbf{97.9} & \textbf{96.6} & 92.1 &	86.9 & 41.2 & 14.9 & 88.9 & 6.1 & \textbf{93.6} & \textbf{87.7}\\
021\_bleach\_cleanser & 88.3 & 48.1 & 36.9 & 16.7 & 89.4 & 44.1 & \textbf{97.4} & \textbf{93.3} & 90.8	& \textbf{85.5} &  5.0 & 2.8 & 89.6 & 32.3 & \textbf{93.0} & 84.6 \\
024\_bowl & 73.2 & 17.4 & 32.7 & 1.4 & 74.7 & 0.9 & \textbf{94.9} & \textbf{89.7} & 87.5	& 43.6 & 3.8 & 3.6 & \textbf{93.2} & 6.7 & 92.1 & \textbf{65.1}\\
025\_mug &  84.8 & 29.5 & 47.3 & 23.6& 86.5 & 39.2 & \textbf{96.2} & \textbf{75.8} &91.0 &	74.1 & 2.6 & 2.6 & 92.5 & 31.6 & \textbf{95.5} &  \textbf{82.9} \\
035\_power\_drill & 60.6 & 12.3 & 18.8 & 1.3 & 73.0 & 19.8 & \textbf{98.0} & \textbf{96.3} & \textbf{97.0}	& \textbf{96.8} &  22.1 & 13.1 & 56.0 & 0.0 & 92.4 & 84.6\\
036\_wood\_block &  70.5 & 10.0 & 49.9 & 1.4 & 94.7 & 27.9 & \textbf{97.4} & \textbf{94.7} & 67.1 &	19.9& 26.3 & 10.5 & 77.1 & 0.0 & \textbf{92.7} & \textbf{85.0}\\
037\_scissors & 75.5 & 25.0 & 32.3 & 14.6  & 74.2 & 27.7 & \textbf{97.8} & \textbf{95.5} &\textbf{97.4}	& \textbf{94.7} & 9.5 & 5.8 & 75.5 & 0.0 & 92.6 & 84.7 \\
040\_large\_marker &81.8 & 38.9 & 20.7 & 8.4 &  97.4 & 74.2 & \textbf{98.6} & \textbf{96.5} & \textbf{92.7} &	90.4& 9.1 & 8.0 & 79.6 & 39.3 & \textbf{96.5}& \textbf{91.0}\\
051\_large\_clamp & 83.0 & 34.4 & 24.1 & 11.2 & 82.7 & 34.7 & \textbf{96.9} & \textbf{92.7} & 87.4 & 68.9 & 22.4 & 8.2 &  \textbf{100.0} &  \textbf{100.0} & 92.9 & 84.2\\
052\_extra\_large\_clamp &  72.9 & 24.1 & 15.0 & 1.8 & 65.7 & 10.1 & \textbf{97.6} & \textbf{94.1} & \textbf{90.5} & 43.7 & 16.9 & 8.1 & 82.6 & 0.0 & 89.5 &  \textbf{65.8}\\
061\_foam\_brick &  79.2 & 35.5 & 59.4 & 31.4 & 95.7 & 45.8 & \textbf{98.1} & \textbf{93.4} & \textbf{98.7}	& 90.9 & 11.3 & 9.1 & 95.2 & 43.5 & 97.6 & \textbf{95.9}\\
\midrule
mean & 71.0 & 24.3 & 52.5 & 26.2 & 88.4 & 42.1 & \textbf{97.4} & \textbf{91.5} & 90.4 &76.1& 13.3 & 7.4 & 86.0 & 25.1 & \textbf{93.7} & \textbf{84.4}\\
         \bottomrule
    \end{tabular}
    \label{tab:ycbv_data_full}
    \vspace{0.2cm}
\end{table*}


\subsection{Full Tracking Results on YCB-Video Sequences}
We present the object tracking results on the full YCB-Video Sequences \cite{xiang2017posecnn} , using the first frame as the reference, in Table \ref{tab:ycbv_tracking_full}. We compare our approach with other CAD model-based novel object pose tracking methods, including \cite{wuthrich2013probabilistic}, RGF \cite{issac2016depth}, ICG \cite{stoiber2022iterative}, and FoundationPose \cite{wen2024foundationpose}. Our method achieves the best performance among one-view-based tracking methods and performs comparably to CAD model-based approaches.

\begin{table*}[]
    \centering
            \footnotesize
        \setlength{\tabcolsep}{2mm}
            \caption{Performance on pose tracking task. We compared with CAD model based tracking methods on YCB-V full video sequences. For our method, we still only give the first frame as a reference, and we keep the reference during tracking.}
    % \vspace{-0.3cm}
    \begin{tabular}{c|c c|c c|c c|c c||c c| c c }
        \toprule
        \textbf{Method}   & \multicolumn{2}{c|}{\textbf{Wuthrich}\cite{wuthrich2013probabilistic}} & \multicolumn{2}{c|}{\textbf{RGF}\cite{issac2016depth}} & \multicolumn{2}{c|}{\textbf{ICG}\cite{stoiber2022iterative}} & \multicolumn{2}{c|}{\textbf{FoundationPose}\cite{wen2024foundationpose}} & \multicolumn{2}{c||}{\textbf{FoundationPose}\cite{wen2024foundationpose}} & \multicolumn{2}{c}{\textbf{One2Any(Ours)}}\\

        Method & \multicolumn{2}{c|}{CAD} & \multicolumn{2}{c|}{CAD}  & \multicolumn{2}{c|}{CAD} & \multicolumn{2}{c||}{16 frames-CAD} & \multicolumn{2}{c|}{$1^{st}$ frame-CAD} & \multicolumn{2}{c}{$1^{st}$ frame} \\
                \midrule
        % Model-based &  \multicolumn{2}{c|}{ \checkmark} & \multicolumn{2}{c|}{ \xmark} & \multicolumn{2}{c|}{ \checkmark} & \multicolumn{2}{c|}{ \xmark} & \multicolumn{2}{c|}{ \xmark} & \multicolumn{2}{c}{ \xmark}\\
        metrics & ADD & ADD-S & ADD & ADD-S & ADD & ADD-S & ADD & ADD-S & ADD & ADD-S &   ADD & ADD-S\\
     \midrule
002\_master\_chef\_can & 55.6 & 90.7 & 46.2 & 90.2 & 66.4 & 89.7  & \textbf{91.2} & \textbf{96.9} & 38.1 &	83.3	& \textbf{83.8} & \textbf{94.8} \\
        003\_cracker\_box & 96.4 & 97.2 & 57.0 & 72.3 & 82.4 & 92.1  & \textbf{96.2} & \textbf{97.5}  & 78.3	& \textbf{94.0}& \textbf{83.0}	& 91.3 \\
        004\_sugar\_box & 97.1 & 97.9 & 50.4 & 72.7 & \textbf{96.1} & \textbf{98.4}  & 94.5 & 97.4 & 40.0	& 78.7 & \textbf{88.7} & \textbf{95.3} \\
        005\_tomato\_soup\_can & 64.7 & 89.5 & 72.4 & 91.6 & 73.2 & 97.3 & \textbf{94.3} & \textbf{97.9} & 14.0	& 49.3&  \textbf{87.1} 	&  \textbf{95.5} \\
        006\_mustard\_bottle   & 97.1 & 98.0 & 87.7 & 98.2 & 96.2 & 98.4 & \textbf{97.3} & \textbf{98.5} & 24.8	& 58.8	 & \textbf{87.7} &  \textbf{93.8}\\
        007\_tuna\_fish\_can  & 69.1 & 93.3 & 28.7 & 52.9 & 73.2 & 95.8  & \textbf{84.0} & \textbf{97.8} & 75.3	&\textbf{ 97.4}	& \textbf{89.5} & 95.9 \\
        008\_pudding\_box & 96.8 & 97.9 & 12.7 & 18.0 & 73.8 & 88.9  & \textbf{96.9} & \textbf{98.5} &\textbf{ 96.9}	&\textbf{98.3} & 93.5	& 96.3\\
        009\_gelatin\_box  & 97.5 & 98.4 & 49.1 & 70.7 & 97.2 & \textbf{98.8} & \textbf{97.6} & 98.5 & \textbf{97.2}	&\textbf{98.6} &  96.1	&97.7 \\
        010\_potted\_meat\_can  & 83.7 & 86.7 & 44.1 & 45.6 & 93.3 & 97.3 & \textbf{94.8} & \textbf{97.5} & 5.5	&52.6 & \textbf{65.9}	&\textbf{84.0}\\
        011\_banana  & 86.3 & 96.1 & 93.3 & 97.7 & \textbf{95.6} & \textbf{98.4} & \textbf{95.6} & 98.1 &64.7&	84.7 & \textbf{ 83.6}	&\textbf{95.1}  \\
        019\_pitcher\_base  & 97.3 & 97.7 & 97.9 & 98.2 & \textbf{97.0} & \textbf{98.8}  & 96.8 & 98.0 & \textbf{94.6}	&\textbf{96.4}	&  87.0 &93.4 \\
        021\_bleach\_cleanser  & 95.2 & 97.2 & 95.9 & 97.3 & 92.6 & \textbf{97.5} & \textbf{94.7} & \textbf{97.5} & 16.6 &	58.6& \textbf{ 84.8} &	\textbf{93.2} \\
        024\_bowl  & 30.4 & 97.2 & 24.2 & 82.4 & 74.4 & \textbf{98.4} & \textbf{90.5} &95.3 & 12.4&	40.2 & \textbf{71.8} &\textbf{91.8}\\
        025\_mug & 83.2 & 93.3 & 60.0 & 71.2 & \textbf{95.6} & \textbf{98.5} &91.5 & 96.1&54.4&	91.3	 & \textbf{83.3} &\textbf{95.5}\\
        035\_power\_drill & 97.1 & 97.8 & 97.9 & 98.3  & 96.7 & 98.5&\textbf{ 96.3} & \textbf{97.9} &50.4	&69.2 & \textbf{85.5} 	&\textbf{92.8} \\
        036\_wood\_block & 95.5 & 96.9 & 45.7 & 62.5 & \textbf{93.5} & \textbf{97.2} & 92.9& 97.0&  \textbf{88.4}	& \textbf{95.9}	& 85.5 &92.8\\
        037\_scissors & 4.2 & 16.2 & 20.9 & 38.6 & 93.5 & 97.3 & \textbf{95.5} & \textbf{97.8} & \textbf{96.0}	&\textbf{97.9} & 81.0	&91.7 \\
        040\_large\_marker & 35.6 & 53.0 & 12.2 & 18.9 & 88.5 & 97.8 & \textbf{96.6} & \textbf{98.6} & 74.0	&90.3 &\textbf{90.3}	&\textbf{96.2}  \\
        051\_large\_clamp  & 61.2 & 72.3 & 62.8 & 80.1 &91.8 &\textbf{96.9} & \textbf{92.5}& 96.7&60.1&	81.0 & \textbf{84.5} & \textbf{93.2} \\
        052\_extra\_large\_clamp  & 93.7& 96.6 & 67.5 & 69.7 & 85.9 & 94.3& \textbf{93.4} & \textbf{97.3}& 44.4	&85.1 & \textbf{71.1}	&\textbf{91.0} \\
        061\_foam\_brick  & 96.8 & 98.1 & 70.0& 86.5 & 96.2 & \textbf{98.5}  & \textbf{96.8} & 98.3 &  89.8&	\textbf{98.2}&	 \textbf{96.1} & 97.7 \\
        \midrule
        mean  & 78.0 & 90.2 & 59.2 & 74.3 & 86.4 & 96.5 & \textbf{93.7} & \textbf{97.5} & 57.9	&80.9	& \textbf{84.8} & \textbf{93.8} \\
        \bottomrule
    \end{tabular}
    \label{tab:ycbv_tracking_full}
    \vspace{0.2cm}
\end{table*}

% \noindent{}\textbf{Pose tracking results on Real275 test set. } We further test the pose tracking performance on Real275 \cite{wang2019normalized}. Results are presented in Table \ref{tab:pose_tracking_nocs}. We compare with Oryon \cite{corsetti2024open} and FoundationPose \cite{wen2024foundationpose} given always the first frame of the test set. Furthermore, we measure the average precision of predicted poses that are with $5\degree5cm, 10\degree5cm$ threshold. Note that, this is a quite strict metrics to measure the pose estimation performance, and we roughly call the poses within the threshold as the 'correct' poses. We tested all 18 objects that belong to 6 categories in Table \ref{tab:pose_tracking_nocs}. We observe that for some objects, FoundationPose failed to estimate the 'correct' poses in bowl, camera, laptop and mugs.


\subsection{Robustness Analysis on the Selection of Reference Images}
To further demonstrate the robustness of One2Any on the selection of different reference images, we additionally measure the standard deviation of the method when dealing with different reference images. We conducted experiments following Oryon~\cite{corsetti2024open}, evaluating 2000 randomly selected reference-query image pairs from the Real275~\cite{wang2019normalized} and Toyota-Light~\cite{hodan2018bop} datasets respectively. These datasets contain various combinations of the same objects
with different reference-query pairs. As shown in Table 1 (main paper), our method significantly outperforms existing approaches when handling different reference images. To further analyze robustness, we computed the standard deviation (std) for each object and averaged
them (see in Table~\ref{tab:different_ref_images}). Our method achieves a lower std, demonstrating its robustness to variations in reference images. 
\begin{table}[]
    \centering
        \footnotesize
        \setlength{\tabcolsep}{3mm}
    \captionof{table}{Robustness Analysis. We measure the standard deviation (std) of AR score and ADD-AUC metrics.}
                % \vspace{-0.3cm}
\begin{tabular}{l | c c | c c}
    \toprule
       \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Real275~\cite{wang2019normalized}} & \multicolumn{2}{c}{Toyota-Light~\cite{hodan2018bop}} \\
         & AR & ADD-AUC & AR & ADD-AUC\\
         \midrule
        % Oryon mean & 46.5 & 34.9 & 34.1 &22.9\\
        Oryon~\cite{corsetti2024open} std & 25.7 & 46.9  & 25.6 & 42.3\\
        \midrule
        % One2Any mean& 54.9 & 41.0 & 42.0 & 34.6 \\
        One2Any std & \textbf{15.6} & \textbf{27.2}  & \textbf{22.5} & \textbf{30.5} \\
        \bottomrule
    \end{tabular}
    \label{tab:different_ref_images}
\end{table}

\subsection{Performance on Occluded Scenes} 
For scenes with occlusions—whether in the reference image or the test image—our method demonstrates strong robustness in handling occluded scenarios, where other methods often fail. Detailed results are presented in Figure \ref{fig:occlusion}.

We observe that occlusions lead to incorrect correspondences in Oryon \cite{corsetti2024open}, causing significant translation errors. This results in a projected pose that is far from the ground truth, as illustrated in row 1, where the predicted pose is projected entirely out of the image. Similarly, NOPE \cite{nguyen2024nope} struggles with occlusions in the reference image. In such cases, suboptimal feature extraction leads to incorrect relative pose predictions in the latent space, as seen in rows 1–3. However, when the reference image provides clear, representative texture input (row 4), NOPE can handle pose estimation effectively, even if the test image is occluded.  FoundationPose \cite{wen2024foundationpose}, on the other hand, heavily depends on the quality of its generated model. Figure \ref{fig:occlusion} shows two views of the generated model: the upper view resembles the reference image, while the lower view corresponds to the test image. When the test view aligns well with the generated CAD model, FoundationPose performs reliably. However, when the test view deviates significantly from the generated model, as seen in rows 2 and 4, it fails to predict the correct pose.

In contrast, our method is highly robust to occlusions in both the reference and test images, consistently achieving accurate pose estimation even under challenging conditions.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{supp_sec/occlusion.pdf}
    \caption{Qualitative results on occluded scenes. We present results for scenarios where occlusion occurs in the reference image and the test image, respectively. The test image displays projected poses with axes, where the green color represents the predicted pose, and the pink color indicates the ground-truth pose. For FoundationPose \cite{wen2024foundationpose}, we also include the generated model derived from the reference image. The upper model view corresponds to the reference image, while the lower model view aligns with the test image. For Oryon \cite{corsetti2024open}, we visualize its predicted correspondences. For One2Any (Ours), we additionally compare the generated ROC map (below) with the ground-truth ROC map (above). }
    \label{fig:occlusion}
\end{figure}

\subsection{Performance on Large View Variations} 
We show qualitative results for scenes with significant view variations in Figure \ref{fig:view_variation}. These scenarios involve objects with markedly different perspectives in the reference and test images. Even in the absence of occlusion, low overlap between the object views presents a significant challenge for pose estimation when only a single reference view is provided.

Methods based on correspondences often fail in such cases due to the difficulty of establishing accurate matches. Similarly, the latent space searching approach used by NOPE \cite{nguyen2024nope} performs poorly when it is unable to conduct a comprehensive search in the latent space. For model-based methods, the effectiveness of the generated model can degrade under such conditions. As shown in the last two rows, only partial regions of the object are generated from the reference image, resulting in poor supervision for pose estimation when the test view has minimal overlap with the reference.

In contrast, One2Any performs robustly even with large view variations. This stability is attributed to the model’s ability to predict ROC maps, effectively inferring missing parts of the object given the Reference Object Embedding (ROPE) and ensuring accurate pose predictions.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{supp_sec/large_view_variation.pdf}
    \caption{Qualitative results on large view variations. We present results for scenarios with significant view variations, including cases with low or almost no overlap between the reference and test images. In the test images, we display the projected poses with axes, where the green color represents the predicted pose and the pink color indicates the ground-truth pose. For FoundationPose \cite{wen2024foundationpose}, we also include the generated model derived from the reference image. The upper view corresponds to the reference image, while the lower view aligns with the test image. For Oryon \cite{corsetti2024open}, we visualize its predicted correspondences. For One2Any (Ours), we additionally show the generated ROC map (below) alongside the ground-truth ROC map (above).}
    \label{fig:view_variation}
\end{figure}
 

\subsection{Performance on Textureless Objects} 
We further present additional results for textureless objects in Figure \ref{fig:textureless}. Textureless objects are known to introduce significant challenges for correspondence matching and template matching methods. As a result, these approaches often fail to predict accurate poses for textureless objects. For example, Oryon \cite{corsetti2024open} struggles with large translation errors, leading to projections that fall outside the image frame.

In contrast, our method, which predicts poses through ROC map generation, demonstrates stability and robustness in handling textureless objects, maintaining accurate pose predictions even under these challenging conditions.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{supp_sec/textureless.pdf}
    \caption{Qualitative results on textureless objects. We evaluate the pose estimation performance for textureless objects, which is presented in Figure \ref{fig:textureless}. The test images display projected poses with axes, where the green color represents the predicted pose and the pink color indicates the ground-truth pose. For FoundationPose \cite{wen2024foundationpose}, we include the generated model derived from the reference image. The upper view corresponds to the reference image, while the lower view aligns with the test image. For Oryon \cite{corsetti2024open}, we visualize its predicted correspondences. For One2Any (Ours), we additionally compare the generated ROC map (below) with the ground-truth ROC map (above).}
    \label{fig:textureless}
\end{figure}

\subsection{More Qualitative Results on Novel Objects}
We present additional qualitative results of our method across various test datasets, including YCB-Video \cite{xiang2017posecnn}, Toyota-Light \cite{hodan2018bop}, T-LESS \cite{hodan2017t}, IC-BIN \cite{doumanoglou2016recovering}, and TUD-L \cite{hodan2018bop}. These datasets are popular in the BOP benchmark. The results are illustrated in Figure \ref{fig:more_visualization}, where we also display the predicted ROC map alongside the reference ROC map.

Our method demonstrates the ability to predict poses for a diverse range of unseen objects across different datasets, such as an unusual toy dinosaur and a charger. Additionally, our method is robust to challenging conditions like significant lighting changes. For instances with large view variations and minimal overlap, such as the cup example, our method accurately estimates the pose.

We also showcase pose tracking performance with the driller object, where our method successfully follows the object’s motion and achieves accurate pose tracking using only the first view as a reference. The processing time is approximately 0.09 seconds per frame with a single Nvidia RTX 4090 GPU.
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{supp_sec/more_visualization.pdf}
    \caption{More qualitative results. We present pose estimation results across additional test datasets, including YCB-Video \cite{xiang2017posecnn}, Toyota-Light \cite{hodan2018bop}, T-LESS \cite{hodan2017t}, IC-BIN \cite{doumanoglou2016recovering}, and TUD-L \cite{hodan2018bop}. For each dataset, we display the ROC maps for the reference images and the predicted ROC maps for the test images. Furthermore, we demonstrate the tracking performance on the YCB-Video dataset. The predicted pose is shown in green, while the ground-truth pose is shown in pink. Additionally, we present the projections of the object point cloud on the image, corresponding to both the ground-truth pose and the predicted pose. }
    \label{fig:more_visualization}
\end{figure}


\subsection{Experiments with RGB-only Inputs} To further explore the ability of One2Any when dealing with RGB query images only (without depth inputs), we use RANSAC+PnP~\cite{fischler1981random}
for pose estimation and tested on YCB-Video~\cite{xiang2017posecnn}. Results are shown in Table~\ref{tab:pose_compute}, we measure the average rotation error and translation error for detailed comparison. RGB-only input achieves competitive rotation estimation, even outperforming Umeyama~\cite{umeyama1991least}. However, estimating translation from a single view without depth is inherently challenging, as depth provides critical scale information. For instance, NOPE~\cite{nguyen2024nope}, a single view method which uses RGB-only input, does not estimate translation at all.

\begin{table}[]
       \centering
    \footnotesize
       \setlength{\tabcolsep}{1.5mm}
      \captionof{table}{Performance of PnP method~\cite{fischler1981random} (without depth input) compared with Umeyama algorithm ~\cite{umeyama1991least} (with depth input). We test on YCB-V test set and measure the rotation error and translation error in detail.}
                       % \vspace{-0.3cm}
    \begin{tabular}{c|c c} % c c}
    \toprule
        Method & rotation err (°) & translation err (m)\\ % & ADD-S & ADD  \\
        \midrule
       Umeyama~\cite{umeyama1991least}  &  22.2 & \textbf{0.02} \\ %& \textbf{93.7} & \textbf{84.4}\\
       RANSAC+PnP~\cite{fischler1981random} &  \textbf{21.0} & 0.04 \\%& 76.4 & 51.6 \\
       \bottomrule
    \end{tabular}
        \label{tab:pose_compute}
\end{table}

\subsection{Training Data Scalability}
\label{sec:training_scale}
We evaluate the impact of training data size on our method. Due to the simplicity of our data collection process—requiring only image pairs of the same object—we can generate an unlimited amount of synthetic data for training. To analyze the effect of training data scale, we gradually increase the size of the training dataset and evaluate performance on the  consistently used test set YCB-Video \cite{xiang2017posecnn}  test set as the evaluation benchmark. The metrics used are ADD-AUC and ADD-S AUC, with results presented in Figure \ref{fig:training_data}.

For comparison, we include performance from FoundationPose \cite{wen2024foundationpose}. Our observations show that the performance of our method improves steadily with an increasing amount of training data. Notably, when the training data size increases to 1M, FoundationPose shows little to no improvement, whereas our method continues to demonstrate significant gains. This indicates that the performance of our approach can be further enhanced with even larger datasets. Due to computational resource limitations, we capped the training data size at approximately 2M samples.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{supp_sec/train_data_scale.pdf}
    \caption{Training data scalability. We analyze the effect of training data size on our method’s performance and compare it with FoundationPose \cite{wen2024foundationpose}.}
    \label{fig:training_data}
\end{figure}


% \begin{table}[]
%     \centering
%         \footnotesize
%         \setlength{\tabcolsep}{0.3mm}
%     \begin{tabular}{c | c |c c |c c | c c}

%                 \toprule
%        & Methods & \multicolumn{2}{c|}{Oryon}  & \multicolumn{2}{c|}{FoundPose}   & \multicolumn{2}{c}{Ours}  \\
%         & Metrics & 5\degree5cm & 10\degree5cm & 5\degree5cm & 10\degree5cm & 5\degree5cm & 10\degree5cm  \\
%         \midrule
%         \multirow{3}{*}{bottle} & 1 & 6.94 & 8.81 & 28.96 & 46.75 & 10.79 & 30.02\\
%         & 2 & 9.71 & 20.38 & 0.00 & 0.00 & 5.73 & 25.48\\
%         & 3 & 2.63 & 14.59 & 25.98 & 34.42 & 11.30 & 36.27\\
%                  \midrule
%         \multirow{3}{*}{bowl}& 4 & 3.97 & 8.83 & 0.19 & 0.19 & 28.92 & 82.56 \\
%         & 5 & 8.30 & 26.11 & 0.00 & 0.00 & 0.00 & 0.00\\
%         & 6 & 6.06 & 12.49 & 2.17 & 9.94 & 2.17 & 15.93\\
%                  \midrule
%         \multirow{3}{*}{camera}& 7 & 9.87 & 26.79 & 0.13 & 0.38 & 17.95 & 39.74 \\
%         & 8 & 9.06 & 25.59 & 0.00 & 0.00 & 16.93 & 59.19\\
%         & 9 & 5.27& 19.02 & 0.00 & 0.00 & 8.74 & 47.94\\
%                  \midrule
%         \multirow{3}{*}{can}& 10 & 1.53 & 3.91 & 56.13 & 73.55 & 5.16 & 39.05 \\
%         & 11 & 0.66 & 0.88 & 56.07 & 93.06 & 8.52 & 36.06\\
%         & 12 & 2.71 & 12.91 & 15.41 & 26.94 & 12.56 & 41.13\\
%                  \midrule
%         \multirow{3}{*}{laptop}& 13 & 30.17 & 49.16 &0.00 & 0.00 & 13.70 & 69.59\\
%         & 14 & 31.62 & 52.73 & 0.00 & 0.00 & 4.95 & 13.43\\
%         & 15 & 29.62 & 45.95 & 0.00 & 0.32 & 11.89 & 30.70\\
%                  \midrule
%         \multirow{3}{*}{mug} & 16 & 7.56 & 16.26 & 0.10 & 0.10 & 28.36 & 75.61\\
%         & 17 & 10.63 & 19.41 & 0.00 & 0.10 & 2.71 & 17.90\\
%         & 18 & 9.02 & 20.15 & 0.00 & 0.00 & 0.19 & 7.49\\
%         \midrule
%         & mean & 11.02 & 22.09 & 10.28 & 16.06 & 9.96 & 35.73\\
%          \bottomrule
%     \end{tabular}
%     \caption{Performance on nocs dataset given only the first view.}
%     \label{tab:pose_tracking_nocs}
% \end{table}

==> supp_sec/3_extension_to_multiview_setups.tex <==
\section{Extension to Multi-view Setups}
\label{sec:multiview_setups}

We further extend our method to multi-view setups. Owing to its time efficiency, our method can seamlessly handle multi-view configurations by estimating the relative pose between the test image and each reference image in the multi-view set. The best prediction is then selected based on these estimations.

\subsection{Simple Voting Strategy for Pose Selection}
Assume we have  $N$  multi-view reference images, resulting in  $N$  predicted poses  $[\mathbf{R}|\mathbf{t}]_{i \in N}$. We employ a simple voting strategy to identify the optimal prediction among these poses.

When utilizing multi-view reference images, we assume low overlap between the images. Consequently, for each test image, there exists an optimal prediction corresponding to one of the reference views. The objective is to use a voting strategy based on reprojection error to identify this best match.


First, we filter out incorrect predictions using reprojection error. Given a predicted relative pose between the test image and reference image  $A_{I_i}$, we estimate the relative pose $[\hat{\mathbf{R}}|\hat{\mathbf{t}}]_{i2r}$, With the ground-truth pose of the reference view $[\mathbf{R}|\mathbf{t}]_{i}$. The predicted pose of the current test image is:
\begin{equation}
    [\hat{\mathbf{R}}|\hat{\mathbf{t}}]_i = [\hat{\mathbf{R}}|\hat{\mathbf{t}}]_{i2r} [\mathbf{R}|\mathbf{t}]_{i}
\end{equation}

Next, we compute the reprojection error from the test image to all reference images. Using the predicted pose, we obtain. We first get the point cloud $W_Q$ in the world coordinate with the predicted pose.
\begin{equation}
    W_Q = {[\hat{\mathbf{R}}|\hat{\mathbf{t}}]_i}^{-1}\mathbf{K}^{-1}Q_D[Q_M=1]
\end{equation}
$\mathbf{K} \in \mathbb{R}^{4\times4}$ is the camera intrinsic matrix, $Q_D, Q_M$ are the depth image and the mask image respectively. Thus, for each reference image $A_j, j\in N$, we have 
\begin{equation}
   P_{A_j} = \mathbf{K}[\mathbf{R}|\mathbf{t}]_{j}W_Q
\end{equation}
Then we get the projected pixels in the image frame
\begin{equation}
        \begin{bmatrix} U \\ V\end{bmatrix}
 = \frac{P_{A_j}[:, :2]}{{P_{A_j}[:, 2]}} 
\end{equation}
And we get the projected mask as:
\begin{equation}
    \hat{A}_{M_j}[U \ V] = 1
\end{equation}
To evaluate the prediction, we compute the mIoU \cite{everingham2010pascal} between the predicted mask $ \hat{A}_{M_j}$ and the ground-truth mask  $A_{M_j}$. Typically, for each test image, there exists at least one reference image where the reprojection results in a high overlap with the ground-truth mask, yielding a high mIoU. However, for other reference images, the predicted mask may result in a lower IoU. Consequently, we select the predicted pose corresponding to the maximum IoU across all reference images as the final predicted pose.
% Thus, we set a threshold to 0.8 that if the IoU is over 0.8, we believe it's a reliable prediction on pose that it correctly project the seen part to one reference image.

% Furthermore, we notice there are some situations that the test image is not like any reference view, resulting its poor mIoU in all reference images. For this case, we simply use a cluster way to find the optimal pose. To be specific, we cluster the predicted poses and find the cluster that has the smallest difference inside, and choose the average pose over the cluster as our prediction.
\begin{table*}[]
\centering
    \footnotesize
    \setlength{\tabcolsep}{0.7mm}
    \caption{Performance on LINEMOD \cite{hinterstoisser2011multimodal} dataset with multi-view setups. We report the recall of ADD-0.1d metric. Results of multi-view methods are taken from FS6D~\cite{wen2024foundationpose}. The best performance among multi-view methods are highlighted in bold. One2Any(Ours) 8-view, 16-view methods are evaluated with a pose selection strategy, while 8-best view and 16-best view results are approached with the best prediction.}
    % \vspace{-0.2cm}
\begin{tabular}{l|c c| c c c c c c c c c c c c c|c}
\toprule
\textbf{Methods} & \textbf{Modality}  & \textbf{Ref. Images} & \textbf{ape} & \textbf{benchwise} & \textbf{cam} & \textbf{can} & \textbf{cat} &  \textbf{driller} & \textbf{duck} & \textbf{eggbox} & \textbf{glue} & \textbf{holepuncher} & \textbf{iron} & \textbf{lamp} & \textbf{phone} & \textbf{mean} \\
% \textbf{Method} & \textbf{ape}    & \textbf{cat} & \textbf{driller} & \textbf{duck} & \textbf{eggbox} & \textbf{glue}   & \textbf{iron} & \textbf{lamp} & \textbf{phone} & \textbf{Avg.} \\
\midrule
% Gen6D \cite{40} & RGB & \xmark & 200 & - & 77 & 66.1 & 62.8 & 60.7 & 67.4 & 40.5 & 95.7 & 87.2 & - & - & - & - & 63.6 \\
% Gen6D \cite{liu2022gen6d} & RGB & 200 & - & 62.1 & 45.6 & 64.7 & 40.9 & 48.8 & 16.2 & - & - & - & - & - & - & - \\
OnePose \cite{sun2022onepose} & RGB & 200 & 11.8 & 92.6 & 88.1 & 77.2 & 47.9 & 74.5 & 34.2 & 71.3 & 37.5 & 54.9 & 89.2 & 87.6 & 60.6 & 63.6 \\
OnePose++ \cite{he2022onepose++} & RGB  & 200 & 31.2 & 97.3 & 88.0 & 89.8 & 70.4 & 92.5 & 42.3 & 99.7 & 48.0 & 69.7 & \textbf{97.4} & \textbf{97.8} & 76.0 & 76.9 \\
LatentFusion \cite{park2020latentfusion} & RGBD & 16 &  \textbf{88.0} & 92.4 & 74.4 & 88.8 & 94.5 & 91.7 & 68.1 & 96.3 & 49.4 & 82.1 & 74.6 & 94.7 & 91.5 & 83.6 \\
% FS6D \cite{he2022fs6d} & RGBD & \xmark & 16 & 74.0 & 86.0 & 88.5 & 86.0 & 98.5 & 81.0 & 68.5 & 100.0 & 99.5 & 97.0 & 92.5 & 85.0 & 99.0 & 88.9 \\
FS6D \cite{he2022fs6d} + ICP & RGBD & 16 & 78.0 & 88.5 & 91.0 & 89.5 & \textbf{97.5} & 92.0 & 75.5 & 99.5 & 99.5 & \textbf{96.0} & 87.5 & 97.0 &\textbf{97.5} & 91.5\\
% FoundationPose \cite{wen2024foundationpose}& RGBD & 16-CAD & \textbf{99.9} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} &  \textbf{100.0} &\textbf{100.0}   & \textbf{99.4} & \textbf{100.0} & \textbf{100.0} & \textbf{99.9} & \textbf{100.0} & \textbf{100.0}& \textbf{100.0} & \textbf{99.9}\\
\midrule 
% % \midrule
% % FoundationPose & RGBD & \xmark & 16 & 99.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 99.4 & 100.0 & 100.0 & 99.9 & 100.0 & 100.0 & 100.0 & \textbf{99.9} \\
% % FoundationPose \cite{wen2024foundationpose}& RGBD & 1-CAD & \textbf{36.5} & \textbf{55.5} & \textbf{84.2} & \textbf{71.7} &  65.3 &16.3  & \textbf{49.8} & 42.6 & 64.8 & \textbf{52.7} & 20.7 & 15.8 & 51.7 & 48.3\\
% % NOPE \cite{nguyen2024nope} & RGB & 1 + GT trans & 2.0 & 4.5 &  2.5 & 2.2 & 0.7 & 4.7& 0.5 &  \textbf{100.0} & 79.4 & 2.9  & 4.5 & 4.2 & 3.9 &16.3\\
% % Oryon \cite{corsetti2024open} &  RGBD & 1 & 1.2 & 1.3 & 3.9 & 0.8 & 12.7  & 8.5 & 0.8 & 63.2 & 18.4 & 1.6 & 0.6 &2.9 & 11.7 & 9.8 \\
% \midrule
% % Ours & RGBD & \xmark & 1 & 43.4 & 59.3 & 59.7 & 59.3 & 54.4 & 65.7 & 35.8 & 100.0 & 99.9&  55.4 & 28.0 & 52.4 & 53.0 &  \\
% One2Any (Ours) & RGBD  & 1 & 33.1& 15.7 & 72.7 & 37.0 & \textbf{66.2}  & \textbf{68.2} & 35.8 & \textbf{100.0} & \textbf{99.9} &  42.0 & \textbf{28.2} & \textbf{31.9} & \textbf{53.2} & \textbf{52.6} \\
\midrule 
One2Any (Ours) & RGBD  & 8 & 79.9 & 75.1 & 88.5 & 60.6 & 90.1 & 70.5 & 45.8 & 100.0 & 99.9 & 84.4 & 60.7 & 84.0 & 89.9 & 79.2\\
One2Any (Ours) & RGBD  & 16 & 82.1 & 85.5 & 92.8 & 75.9 & 94.1 & 80.4 & 65.9 & 100.0 & 99.9 &  70.7 & 61.7 & 91.5 & 84.1 & 83.7  \\
\midrule
% One2Any (Ours) & RGBD  & 4-best view \\
One2Any (Ours) & RGBD  & 8-best view & 85.0 & 93.7 & 97.8 & 84.9 & 94.9 & 90.1 & 73.2 & 100.0 & 99.9 & 88.8 & 89.8 & 95.4 & 85.2 & 90.7\\
One2Any (Ours) & RGBD  & 16-best view & 84.8 & \textbf{98.3} & \textbf{98.8} & \textbf{95.2} & 95.9 & \textbf{93.3} & \textbf{76.2} & \textbf{100.0} & \textbf{99.9} & 92.9 & 95.1 & 94.4 & 93.9 & \textbf{93.8}\\

% FoundPose \cite{wen2024foundationpose} &36.5  &  65.3  & 49.8 & 42.6 & 99.0 & 64.8 & 20.7 & 15.8 & 51.7 & 49.6\\
% NOPE \cite{nguyen2024nope}  & \\
% Oryon \cite{corsetti2024open} & 1.2  & 85.2 & 0.3  & 0.8 & 63.2 & 18.4 & 1.6  &2.9 & 11.7 &   20.6\\
% \midrule
% % Ours & RGBD & \xmark & 1 & 43.4 & 59.3 & 59.7 & 59.3 & 54.4 & 65.7 & 35.8 & 100.0 & 99.9&  55.4 & 28.0 & 52.4 & 53.0 &  \\
% Ours & 33.1  & 66.2  & 68.2 & 35.8 & 100.0 & 99.9&  28.2 & 31.9 & 53.2 & 57.4\\
\bottomrule
\end{tabular}
    \label{tab:multi-view}
\end{table*}

\subsection{Experiments with Multi-view Setups}
We conduct experiments on the challenging LINEMOD dataset \cite{hinterstoisser2011multimodal}, which features significant view variation. Results are presented in Table \ref{tab:multi-view}. In addition, we evaluated the performance of our method with 8 /16  reference views. Using the simple pose selection strategy, our method achieved a 50\% improvement with 8 reference views and a 59\% improvement with 16 reference views. Notably, the performance with 16 reference views surpasses LatentFusion \cite{park2020latentfusion}, which learns an object latent space to render additional views. While FS6D \cite{he2022fs6d} is specifically fine-tuned for the LINEMOD dataset, OnePose \cite{sun2022onepose} and OnePose++ \cite{he2022onepose++} require over 200 reference views to compensate for the lack of depth information but still perform poorly.

However, the simple selection strategy does not always guarantee the optimal predicted pose. To address this, we further analyze the best-case prediction results (last two rows of Table \ref{tab:multi-view}),where the predictions most closely resemble the ground truth. These results show significant improvements, demonstrating that our method outperforms many existing multi-view approaches. 

Furthermore, the experimental results demonstrate that our method has the potential to be further enhanced and explored in multi-view setups, offering even greater capabilities.

% \begin{table*}[]
%     \centering
%     \footnotesize
%        \setlength{\tabcolsep}{0.2mm}
%     \caption{Performance on occluded YCB-Video \cite{xiang2017posecnn} dataset. We compare with point cloud registration methods, multi-view methods, and one-view methods. Predator \cite{huang2021predator}, LoFTR \cite{sun2021loftr} and FS6D \cite{he2022fs6d} are fine-tuned on the YCB-Video dataset. We evaluate ADD-S AUC and ADD AUC metrics. Results of multi-view methods are adopted from \cite{wen2024foundationpose}. For one-view methods, we provide the first image in the test set as the reference. The best performance among multi-view methods and one-view methods are highlighted in bold.}
%     \begin{tabular}{c| c c | c c |c c |c c ||c c | c c | c c | c c}
%     \toprule
%         Methods  &\multicolumn{2}{c|}{\textbf{PREDATOR} \cite{huang2021predator}} & \multicolumn{2}{c|}{\textbf{LoFTR}\cite{sun2021loftr}} &  \multicolumn{2}{c|}{\textbf{FS6D} \cite{he2022fs6d}} & \multicolumn{2}{c||}{\textbf{FoundationPose} \cite{wen2024foundationpose}} &  \multicolumn{2}{c}{\textbf{One2Any(Ours)}} &  \multicolumn{2}{c}{\textbf{One2Any(Ours)}}  &  \multicolumn{2}{c}{\textbf{One2Any(Ours)}} & \multicolumn{2}{c}{\textbf{One2Any(Ours)}} \\
  
%         Ref. Images & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{16 - CAD}  & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{8} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c}{1} \\
%         \midrule
%         metrics & ADD-S & ADD & ADD-S & ADD  & ADD-S & ADD  & ADD-S & ADD & ADD-S & ADD & ADD-S & ADD & ADD-S & ADD & ADD-S & ADD \\
%         \midrule
%        002\_master\_chef\_can  &73.0 & 17.4 & 87.2 & 50.6& 92.6 & 36.8 & \textbf{96.9} & \textbf{91.3} & & \textbf{94.9} & \textbf{84.3}\\
% 003\_cracker\_box & 41.7 & 8.3 & 71.8 & 25.5  & 83.9 & 24.5 & \textbf{97.5} & \textbf{96.2} &  & 91.1 & \textbf{83.3}\\
% 004\_sugar\_box &  53.7 & 15.3 & 63.9 & 13.4 & 95.1 & 43.9 & \textbf{97.5} & \textbf{87.2} &  & \textbf{95.3} &\textbf{88.0} \\
% 005\_tomato\_soup\_can & 81.2 & 44.4 & 77.1 & 52.9 & 93.0 & 54.2 & \textbf{97.6} & \textbf{93.3} & & 93.6 & 80.9 \\
% 006\_mustard\_bottle &  35.5 & 5.0 & 84.5 & 59.0&  97.0 & 71.1 & \textbf{98.4} & \textbf{97.3} &  & \textbf{93.8} & \textbf{87.6}\\
% 007\_tuna\_fish\_can &  78.2 & 34.2 & 72.6 & 55.7 & 94.5 & 53.9 & \textbf{97.7} & \textbf{73.7} &  & \textbf{95.9} & \textbf{90.0}\\
% 008\_pudding\_box &  73.5 & 24.2 & 86.5 & 68.1& 94.9 & 79.6 & \textbf{98.5} & \textbf{97.0} & & \textbf{96.1} & \textbf{93.3} \\
% 009\_gelatin\_box &  81.4 & 37.5 & 71.6 & 45.2 & 98.3 & 32.1 & \textbf{98.5} & \textbf{97.3} &  & \textbf{97.7} & \textbf{96.1}\\
% 010\_potted\_meat\_can &  62.0 & 20.9 & 67.4 & 45.1 & 87.6 & 54.9 & \textbf{96.6} & \textbf{82.3} & & 86.3 &  72.5\\
% 011\_banana &  57.7 & 9.9 & 24.2 & 1.6 & 94.0 & 69.1 & \textbf{98.1} & \textbf{95.4} & & \textbf{95.0} & \textbf{85.7}\\
% 019\_pitcher\_base &  83.7 & 18.1 & 58.7 & 22.3 & 91.1 & 40.4 & \textbf{97.9} & \textbf{96.6} &  & \textbf{93.6} & \textbf{87.7}\\
% 021\_bleach\_cleanser & 88.3 & 48.1 & 36.9 & 16.7 & 89.4 & 44.1 & \textbf{97.4} & \textbf{93.3} &  & \textbf{93.0} & 84.6 \\
% 024\_bowl & 73.2 & 17.4 & 32.7 & 1.4 & 74.7 & 0.9 & \textbf{94.9} & \textbf{89.7} &  & 92.1 & \textbf{65.1}\\
% 025\_mug &  84.8 & 29.5 & 47.3 & 23.6& 86.5 & 39.2 & \textbf{96.2} & \textbf{75.8} & & \textbf{95.5} &  \textbf{82.9} \\
% 035\_power\_drill & 60.6 & 12.3 & 18.8 & 1.3 & 73.0 & 19.8 & \textbf{98.0} & \textbf{96.3} & & 92.4 & 84.6\\
% 036\_wood\_block &  70.5 & 10.0 & 49.9 & 1.4 & 94.7 & 27.9 & \textbf{97.4} & \textbf{94.7} &  & \textbf{92.7} & \textbf{85.0}\\
% 037\_scissors & 75.5 & 25.0 & 32.3 & 14.6  & 74.2 & 27.7 & \textbf{97.8} & \textbf{95.5} & & 92.6 & 84.7 \\
% 040\_large\_marker &81.8 & 38.9 & 20.7 & 8.4 &  97.4 & 74.2 & \textbf{98.6} & \textbf{96.5} &  & \textbf{96.5}& \textbf{91.0}\\
% 051\_large\_clamp & 83.0 & 34.4 & 24.1 & 11.2 & 82.7 & 34.7 & \textbf{96.9} & \textbf{92.7} &  & 92.9 & 84.2\\
% 052\_extra\_large\_clamp &  72.9 & 24.1 & 15.0 & 1.8 & 65.7 & 10.1 & \textbf{97.6} & \textbf{94.1} & & 89.5 &  \textbf{65.8}\\
% 061\_foam\_brick &  79.2 & 35.5 & 59.4 & 31.4 & 95.7 & 45.8 & \textbf{98.1} & \textbf{93.4} &  & 97.6 & \textbf{95.9}\\
% \midrule
% mean & 71.0 & 24.3 & 52.5 & 26.2 & 88.4 & 42.1 & \textbf{97.4} & \textbf{91.5} & & \textbf{93.7} & \textbf{84.4}\\
%          \bottomrule
%     \end{tabular}
%     \label{tab:ycbv_data_full}
% \end{table*}
